Transformers Learn Two Competing Sorting Algorithms, and Only One Length-Generalizes

We show that two-layer transformers trained to near-zero loss on a sorting task converge to one of two mechanistically distinct solution classes depending on their initialization. One solution class consists of solutions that do not use the second attention layer to sort, but also fail to length-generalize. The other, which uses both attention layers, length-generalizes perfectly, despite only being trained to sort sequences of a fixed length. By carefully choosing the weight initialization, we demonstrate that we can steer the model toward learning one solution or the other. We identify input types that are rare at the training length but increasingly common at longer sequence lengths as a source of this disparity in length-generalization, and find that layer-wise specialization of the second class of solutions allows them to handle these rare sequences more accurately. In the second class, we discover a mechanism by which the second layer attention can use the contextual information gathered by the first layer attention to reduce its search space. On the related task of finding the minimum of a sequence, we find a similar two solution-type phenomenon, but with the opposite generalization pattern, where a different form of layer-wise specialization causes the two-layer solution to length-generalize worse than the single-attention solution.

==> sections/abstract.tex <==
We show that two-layer transformers trained to near-zero loss on a sorting task converge to one of two mechanistically distinct solution classes depending on their initialization. One solution class consists of solutions that do not use the second attention layer to sort, but also fail to length-generalize. The other, which uses both attention layers, length-generalizes perfectly, despite only being trained to sort sequences of a fixed length. By carefully choosing the weight initialization, we demonstrate that we can steer the model toward learning one solution or the other. We identify input types that are rare at the training length but increasingly common at longer sequence lengths as a source of this disparity in length-generalization, and find that layer-wise specialization of the second class of solutions allows them to handle these rare sequences more accurately. In the second class, we discover a mechanism by which the second layer attention can use the contextual information gathered by the first layer attention to reduce its search space.
%\khasha{@nathan i tried to write this closer to your initial proposal, a bit more conservative.}\nathan{I agree with this a lot more. Thanks. Can I just suggest changing it to "the second layer attention can use the contextual information" where we change "uses" to "can use" since the phenomenon depends on the two-stage seed and the token?}\khasha{yes i agree can use is better}
On the related task of finding the minimum of a sequence, we find a similar two solution-type phenomenon, but with the opposite generalization pattern, where a different form of layer-wise specialization causes the two-layer solution to length-generalize worse than the single-attention solution.

==> sections/alternate_algorithms.tex <==
\section{How well do these phenomena persist across other algorithms?}\label{sec:alternate_algorithms}

%\nathan{I think we should move this section higher up so that the figures match better}

While this paper has focused on sorting, where the split between solution types is cleanest, the phenomenon is not specific to sorting. We also study two related tasks that are possible to implement with a single transformer layer, but train them using the same two-layer architecture. Across these tasks, we again find that different initialization seeds lead to solutions that differ in the extent to which they use the second attention layer. We also find that the solution type predicts length-generalization. However, the relationship between using the second layer and length-generalization is not the same across tasks.

The three tasks we study are closely related conceptually. Sorting repeatedly finds the next larger element in the input, while minimum-finding performs only the first step of this procedure and greedy coin denomination repeatedly finds the largest denomination that does not exceed the current remainder and deducts it from the remainder. Thus, sorting and coin denomination both involve successor or predecessor queries, which only require one layer of a transformer to perform. Despite these similarities, the three tasks produce different distributions of solution types and different patterns of length-generalization.

\paragraph{Minimum-finding.}
We train the same two-layer architecture to find the minimum of a length-$K$ sequence of integers drawn from ${1,\ldots,N}$ with replacement. The input consists of the sequence followed by a separator token, and the model outputs the minimum value. We train at $K=16$ with $N=4096$ and evaluate at longer sequence lengths.

One important distinction between the sorting task and the minimum-finding task is that for the minimum-finding task, we sample input sequences with replacement. Sorting with duplicates cannot be performed by a single attention layer without positional encodings, since the model must keep track of how many copies of each value to output. Minimum-finding, in contrast, remains possible with one layer because the output does not depend on a value's multiplicity. This is why minimum-finding lets us compare single-stage and two-stage solutions while allowing inputs with duplicates.

\paragraph{Greedy coin denomination.}
We also study the task of greedy coin denomination. The input is a set of distinct denominations, followed by a separator token and a target value. The model must output the sequence of remainders produced by repeatedly subtracting the largest denomination that does not exceed the current remainder. We train on denomination sets of size $K=8$ and evaluate on larger sets.
This task is closely related to sorting because at each output step, the model must find the largest available denomination below the current remainder. This is a predecessor query, whereas sorting requires a successor query. We study the greedy algorithm rather than the optimal change-making algorithm since it is an easier task that can be done with a single layer transformer. However, it is not optimal for every set of denominations.

For both tasks, we choose the vocabulary size scale so that the vocabulary size is small enough for a single-stage solution to be learnable, but large enough that the model sometimes learns to use the second layer. Since minimum-finding, is easier than sorting, we use a larger vocabulary for minimum-finding ($N=4096$, compared with $N=256$ for sorting) before two-stage solutions appear at appreciable rates. We then choose a symmetric initialization scale at which both solution types occur at similar rates. For minimum-finding, we use $\sigma=0.006$, selected from a scan over $\sigma\in[0.005,0.01]$; for coin denomination, we use $\sigma=0.1$.

\subsection{Different tasks produce different solution types}
Figure~\ref{fig:three-tasks} shows the results for all three tasks. As with sorting, ablating the second attention layer separates models according to how much they use the second layer. Some models are almost completely unaffected by the ablation, indicating that they have learned a single-stage solution. Other models fail after the ablation, indicating that they use both attention layers.
For sorting, the two-stage models length-generalize better than the single-stage models. Greedy coin denomination shows the same overall pattern where models that rely more on the second attention layer tend to generalize better, although the solutions form a more continuous range than they do for sorting.
Minimum-finding shows the opposite pattern where the single-stage models generalize better than the two-stage models. Thus, we emphasize that the relationship between solution types and length-generalization is a property of the task.

\subsection{Competing failure modes in minimum-finding}

The minimum-finding result can be understood by comparing the adversarial examples of the two solution types. Both solution types achieve high accuracy at the training length, but they fail on different types of inputs. In particular, two-stage models degrade when many input values are close to the minimum. These inputs are rare at the training length, but become increasingly common as the sequence length grows. Single-stage models are more robust to these inputs, but are less robust to examples involving duplicate numbers than two-stage models.

One hypothesis is that duplicates are difficult because they require more precise attention scores. Suppose the minimum has pre-softmax score $a_1$, while each of $n$ copies of the second-smallest value has score $a_2$. To place more total attention on the minimum, the model needs $e^{a_1} > n e^{a_2}$, or equivalently $a_1-a_2 > \log n$. 
Thus, the required score margin grows with the number of copies of a competing value. The additional layer in the two-stage models may help make these distinctions. This would explain why they handle some duplicate-related inputs better, but fail on crowded near-minimum inputs.

These results suggest that length-generalization depends on how the failure modes of a learned algorithm interact with changes in the input distribution. In sorting, the two-stage solution handles small-gap inputs, which become more common at longer lengths. In minimum-finding, the two-stage solution instead appears to fail on inputs with many values close to the minimum, while performing better on some inputs involving duplicates. More generally, additional expressivity may help a model handle some input types that are rare at the training length and whether this improves length-generalization depends on whether those input types become important at longer lengths. Studying the minimum-finding and coin denomination solutions in more depth, and building a more general understanding of how and when this occurs is an interesting direction we leave for future work.

==> sections/introduction.tex <==
\section{Introduction}

\iffalse
\nathan{Some general to-dos:
- make plots more readible. Both making text bigger and also thinking about more effective ways to convey the same information than the current format we have

- check consistency with citep, cite, etc.

- general time spent on editing, to make the writing quality good

- remember to add a bit in the appendix about deeper models
}
\fi

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figures/combined_two_types_binhalf.pdf}
  \caption{\textbf{Across three tasks possible to implement with a single transformer layer, two-layer transformers learn multiple solution types when the initializations are varied, and length-generalization abilities depend on the solution type.} Each curve is one trained model's \emph{token accuracy}, evaluated beyond its training length, colored by its sequence accuracy when the second attention layer is ablated (its
\emph{removability}, summarized in the side histograms, showing the distribution of removability across seeds). \textcolor{red}{Single-stage} models are unaffected by the ablation, while \textcolor{blue}{two-stage} models have poor accuracy without the second attention layer. \textbf{(a)}~ \textbf{Sorting}, the accuracy after ablating the second attention is either 0 or 1 depending on the seed, and \textcolor{blue}{two-stage} solutions length-generalize almost perfectly while \textcolor{red}{single-stage} solutions length-generalize poorly. \textbf{(b)}~ In the \textbf{minimum-finding} task, the pattern reverses where \textcolor{red}{single-stage} solutions generalize better than \textcolor{blue}{two-stage} solutions (which happen to be more common at larger initialization scales). \textbf{(c)}~ In the \textbf{greedy coin denomination} task, the same pattern as sorting occurs but with a broader, less bimodal spread, and a weaker correlation between being a \textcolor{blue}{two-stage} solution and generalizing better. In every case both types are perfect in-distribution, yet which one length-generalizes is task-dependent.}
  \label{fig:three-tasks}
\end{figure}

A recurring hope in mechanistic interpretability is that neural networks trained on well-understood tasks will rediscover familiar algorithms, and that similar mechanisms will recur across independently trained models \citep{olah2020zoom, akyürek2023learningalgorithmincontextlearning}. Recent work has complicated this picture by demonstrating settings in which neural networks can implement one of multiple solutions to the same task. 

For modular addition, \citep{zhong2023clock} identified two mechanistically different solutions, termed the ``Clock'' algorithm and the ``Pizza'' algorithm, and showed that changes in architectural hyperparameters can determine which solution emerges. This line of work was later extended to other tasks with multiple training outcomes, including learning mixtures of markov chains \citep{park2024competition} \citep{wurgaft2025context}, state tracking \citep{li2025howlanguagemodelstrack}, and algorithmic tasks such as counting and addition \citep{zhao2025random}, where different solutions also have different generalization behavior OOD or at longer lengths. Building on these results, our paper introduces a more general setting for studying when neural networks converge to one of two qualitatively different solutions. In particular, we study tasks that are possible for a one-layer transformer to implement, and train them with a two-layer transformer. 
%Authors in~\cite{park2024competition} further show that the circuits implementing the length-generalizable algorithm—which uses in-context learning to predict the next state of a Markov chain—emerge and later disappear during training, suggesting that there is a sweet spot in the number of training steps.   

% \nathan{(Note to say a bit more about the state tracking paper, since it is so similar to ours.)} % actually, maybe it's fine as is

While common intuition about training dynamics suggests that neural networks have a "simplicity bias" where they tend to converge to simpler solutions, and that simpler solutions generalize better than complex ones~\citep{pmlr-v235-gatmiry24a,du2024hierarchicalsimplicitybias,shah2020pitfalls}, recent work refutes this conventional wisdom~\citep{pmlr-v235-tsoy24a}. Our set-up provides explicit examples challenging this intuition.\khasha{this previous sentence has to prob be removed} We find that under some parameter initializations, these two layer transformers converge to single-layer solutions, where the second attention can be ablated without impacting accuracy, while for other initializations, the transformers converge to a solution that meaningfully uses both layers. We find that for the task of \emph{minimum-finding}, the simpler single-layer solutions generalize better. However, for the task of \emph{sorting numbers}, we find that the more complex two-layer solutions generalize better, counter to common intuition about simplicity bias. In a third, \emph{greedy coin denomination} task, we find a larger variation in types of solutions learned, and more mixed results about generalization, but with a correlation between reliance on the 2nd attention layer and length-generalization abilities.

This paper focuses on the task of sorting numbers, where we find the cleanest split in solution types across seeds. We study this task in more detail with mechanistic interpretability, aiming to explain the unintuitive phenomenon of the more complex 2-layer solution length-generalizing better. Sorting a sequence of numbers is a task in $\mathbf{FTC^{\mathrm{0}}}$ which can theoretically be performed with just a single layer transformer given a large enough embedding size. In fact, authors in~\citep{weiss2021thinking} show that training a single layer transformer for sorting reaches accuracy close to one.  

In particular, we argue for two mechanisms of why length-generalization occurs in the more complex solution. First, the more complex solution learns a form of cross-layer specialization to more accurately sort sequences with many consecutive numbers: a property that is rare at the length trained at, but increasingly common at longer evaluation lengths. Second, we show evidence of a hinting mechanism, where the first layer can provide a range of possible next tokens to the second, making it easier to select the correct next token out of a candidate set of potential next tokens that grows with larger input lengths. We additionally show how to steer the model toward each solution type by varying the initialization scale across layers.

\textbf{Organization.} Section~\ref{sec:setup} introduces the task and experimental setup.
Section~\ref{sec:two-algorithms} presents the two solution types and describes each at a high level.
Section~\ref{sec:mechanistic} gives a mechanistic analysis of the two-stage solution, identifying two properties that account for its length-generalization advantage. Section~\ref{sec:steering} investigates what determines which algorithm emerges from training. In the final section, we discuss results for algorithms other than sorting.



==> sections/mechanistic.tex <==
%\section{Mechanistic Analysis of Two-stage Solutions}
%\label{sec:mechanistic}

We identify two properties of the two-stage solution that may account for its superior length-generalization. First, the two attention layers specialize across gap sizes between consecutive tokens, where the first layer handles tokens with small gaps to the next largest number, while the second layer has a larger role for tokens where the gap to the next largest token is larger (\S\ref{sec}). Importantly, sequences with small gap sizes lie in the low-probability tail of the training distribution at small training lengths, so a model can achieve high overall accuracy without handling them reliably. However, as sequence length increases, the gap distribution shifts toward smaller values, making this previously rare statistic increasingly likely. Correctly handling small gaps therefore becomes increasingly important for length-generalization. Second, we provide evidence that the first attention layer can supply the second with contextual information that narrows the search for the correct next token to a smaller interval (\S\ref{sec}). This \emph{windowed monotonicity} mechanism may be another factor that allows the second attention layer to maintain a sharp, accurate attention distribution even as sequence length grows and tokens become more densely packed.

\subsection{Handling Rare Sequences With Specialization Across Layers}
\label{sec:specialization}

While single-stage solutions to the sorting task are measured to have perfect accuracy, we find that they still have adversarial examples. For example, input sequences that are permutations of consecutive integers, with gaps of $1$ between sorted input tokens, are unable to be sorted by single-stage models, but can be sorted by two-stage models. As sequence length grows, sequences with smaller gap sizes between tokens become increasingly likely. As we reach an input length equal to the vocabulary size, every gap becomes exactly 1, which we know single stage models are unable to sort, even at short sequence lengths. We hypothesize that the high accuracy of two-stage models on these rare sequences is enabled by a form of layerwise specialization, where tokens of small gaps (whose next largest token is close) are generally handled mostly by the first layer, while predicting large token gaps is handled more by the second layer's attention. We present three pieces of evidence supporting this layerwise specialization hypothesis in this subsection.

\paragraph{The first attention provides weaker contextual information at large gaps.}
Figure~\ref{fig:specialization_across_layers} demonstrates that as the token gap increases, the first attention increasingly attends to tokens outside the input sequence, either attending to the separator token, which may act as an attention sink, or to tokens in the already-sorted output, which cannot contain values larger than the current token. At large gaps, the first attention attends very weakly to input tokens, suggesting that the amount of contextual information the first layer provides may diminish as the gap grows.

\paragraph{The first layer often suffices at small gaps.}
Conversely, for most seeds, removing the second attention does not impact the token accuracy at small gap sizes (Figure~\ref{fig:removal_of_l2_by_gap}), suggesting that the "two-stage" nature of the two-stage solution type mostly applies when predicting tokens at large gaps. At the same time, although we distinguish between single-stage and two-stage solutions as two families of mechanisms, the varying results across seeds in this experiment also demonstrates that there is wide variation in algorithms within the two-stage family, particularly regarding how responsibility is distributed across layers.

\begin{figure}[!t]
  \centering

  \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]
      {arxiv/figures/fig4a_attention_on_input.pdf}
    \phantomcaption
    \label{fig:specialization_across_layers}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]
      {figures/fig4b_ablation_by_gap.pdf}
    \phantomcaption
    \label{fig:removal_of_l2_by_gap}
  \end{subfigure}

  \caption{\textbf{(a)}~Fraction of the first attention's mass on input-sequence tokens as a
    function of gap size, averaged over two-stage models. As the gap increases,
    the first attention increasingly attends to the separator token or sorted-output tokens
    rather than unsorted input tokens, indicating that the first attention may be playing a less significant role in the computation.
    \textbf{(b)}~Token accuracy after removing the second attention, broken down by gap size,
    across two-stage seeds. For many two-stage seeds, even though the accuracy on random inputs goes to 0 after removing the 2nd attention, for tokens of gap size 1, the accuracy remains at $100\%$ after the ablation. However, for some of the two-stage seeds, however, accuracy drops even at gap~$1$, indicating reliance on the second layer at all gap sizes. which is corroborated by Figure~\ref{figures/hijack_allI_avg_seeds_fl.png}.} % \nathan{Want to say something like: Most two-stage models have perfect accuracy without the 2nd layer at small gaps, but there are some outliers where the second layer plays a larger role at all gaps. (should also emphasize in the text that at larger lengths, the gap shrinks, meaning that some seeds can sort at long lengths even without using the 2nd layer (then reference experiment for this in the appendix).}
  \label{fig:gap-specialization}
\end{figure}

\paragraph{Gap-dependent specialization across layers.}

We corroborate the layerwise division of labor at different gap sizes with two causal interventions. We perform a \emph{direct circuit intervention} by forcing the first attention layer to attend to a chosen token, but apply this redirection only to the pathway that bypasses the second attention, while leaving the first attention’s input to the second attention unchanged. We define the \emph{hijack success rate} as the percentage of interventions for which the model’s prediction changes to the chosen token. In the second intervention, we force the second attention layer to attend to a chosen token and also measure the hijack success rate. Figure~\ref{fig:hijack-fl-avg} reports the mean hijack success rates of both interventions across six gap sizes, averaged over 23~two-stage seeds with sequence length~$32$ and vocabulary size~$512$. At the smallest gap, both hijacks succeed at fairly significant rates, but with a very large spread across seeds, similar to the spread seen in Figure~\ref{fig:removal_of_l2_by_gap}. The co-success rate is approximately 20\%, indicating that both pathways can influence the model's prediction. As the gap grows, the first attention's direct circuit loses influence, while the second attention hijack success rate remains close to $100\%$ across all gaps, corroborating results found in Figure~\ref{fig:specialization_across_layers}.

% \nathan{When I think more about it, the take away at small gaps here feels contradictory to the take away in the previous subsection. An explanation that would be consistent with both results is as follows: even in situations where one can remove the 2nd attention, what it attends to still tends to follow the first attention if the first attention is confident (i.e. attending strongly to the input sequence as in figure 3a), and as a result, it seems reasonable that the final output could either be read off of the first attention or the second attention or a combination, regardless of whether the first attention is "doing the work". As a result, I have a bit of an issue with the take away at small gaps. I think the take away at large gaps makes a lot of sense, but I really think we should be careful about how we interpret results at gap size 1 to not make incorrect claims.} 
% \khasha{I added a sentence above on this, I think we have a good understanding of small gap story from the later descriptions and hijacking experiments: either layer 1, or layer 2, or both layers at the same time could be responsible for the small gaps}

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]%{figures/hijack_allI_avg_seeds_fl.png}
{figures/hijack_allI_avg_seeds_fl_v3_paper_large_seeds.png}
  \caption{Hijack success rates averaged over all values of~$i$ and 23~two-stage
    seeds (sequence length $32$, vocabulary size $512$). Each panel shows a different gap~$g$. Red:
    redirecting the first attention's direct circuit (bypassing the second attention). Blue: redirecting
    the second attention's focus. Purple (dashed): fraction of instances where both
    interventions independently succeed on the same input. At small gaps, both
    circuits contribute, to varying extents depending on the seed; as the gap grows, the second attention dominates entirely. \nathan{As this is the only experiment with vocab size 512, I am concerned that readers will perceive this as cherry-picking.}}
  \label{fig:hijack-fl-avg}
\end{figure}

\subsection{How the first attention can assist the second}
\label{sec:attn2-qk-mechanism}

While at very small or very large gaps the two-stage model primarily specializes across layers, we believe that at intermediate gaps, common at the training length or medium-long context, both layers play a compositional role in predicting the next token. In this section we describe how we believe the first layer can provide contextual input to the second and how this may assist with length generalization at intermediate lengths.

Figure~\ref{fig:ridgeline} (top left) shows that the first attention layer produces a coarse estimate of the next sorted token. In particular, while the first attention often attends most strongly to the correct next token, sometimes it makes an error. The second attention layer then makes this estimate more accurate attending more frequently to the correct next token than the first layer (Figure~\ref{fig:ridgeline}, top right). Quantifying this, the token that the second attention attends to most matches the correct next token ${\approx}99.5\%$ of the time, compared to ${\approx}86\%$ for the first attention.

We explain the accuracy gap between the two attention layers with a hinting mechanism:
attention layer 1 supplies attention layer 2 with contextual information that effectively provides an \emph{upper bound} on the next correct number. This hint originates from the query side, where the first attention gathers contextual information about the current output position and passes it forward through the residual stream, giving the second attention an estimate of where the next sorted value lies. The second attention then uses this signal to
adjust the current token's representation so that its attention is concentrated
on the narrow range between the current value and the upper bound provided by
the first attention, rather than searching over the entire vocabulary. Next, we elaborate on the purpose and impact of this representation adjustment used by the second attention with the contextual information provided by the first. 
%%
This mechanism is, in essence, a divide-and-conquer strategy that the model acquires, although its implementation differs substantially from that of classical sorting algorithms.

%\khasha{Add comparison on algorithmic interpretation of these types and emphasize on divide an conquer strategy here}

As a technical detail, we find that the second attention's QK scores depend almost exclusively
on the first MLP's output rather than the full residual stream: replacing the second attention's input
with the first MLP's output alone causes negligible changes in both the attention
distribution ($\ell_1$ distance $< 0.03$) and full-model accuracy (maximum
drop $0.05\%$) across 13 of 15 two-stage checkpoints that were trained with random initializations different from one another.
(Appendix~\ref{app:attn2-mlp1-dependence}). This allows us to
analytically characterize the second attention score as a function of four quantities: the
query token~$z$, the key token~$t$, the first attention target on the query side~$x$,
and the first attention's target on the key side~$y$:
\[
  s(z, x, t, y)
  \;=\;
  \mathbf{q}(z, x)^\top \mathbf{k}(t, y),
\]
where $\mathbf{q}(z,x) = W_Q^{(2)} \operatorname{LN}\!\bigl(
\operatorname{MLP}_1\!\bigl(\operatorname{LN}(e_z + V^{(1)}_x)\bigr)\bigr)$
and $\mathbf{k}(t,y)$ is defined analogously. Here $V^{(1)}_x$ denotes the
first-layer attention's value vector for token~$x$ (projected through $W_O^{(1)}$).
%%
Figure~\ref{fig:qk-heatmap-asymmetry} plots the score as a heatmap while
varying either the key-side target~$y$ (middle) or the query-side target~$x$
(right), with the other variables held fixed at $z = 250$. The middle panel
shows nearly uniform horizontal bands---the score depends on the key
\emph{token}~$t$ but is essentially invariant to which token the first attention attended on
the key side. In contrast, the right panel exhibits rich structure: as the
query-side target~$x$ increases, a high-score band emerges in the interval
$[z, x]$, and the argmax shifts to track~$x$. This demonstrates that
\textbf{the second attention uses contextual information from the first attention exclusively on the query
side}, consistent with the hinting mechanism described above.

\textbf{Windowed monotonicity.}
Crucially, due to the existence of the hint gathered by the first-layer attention, the second attention does not need to learn a globally
correct ranking over the entire vocabulary  to achieve high prediction accuracy---it only needs to rank tokens
correctly within the narrow window $[z, x]$ defined by the current value~$z$
and the upper-bound hint~$x$ from the first attention. This is the key insight explaining
why the second attention can be dramatically more accurate than the first despite inheriting its
information: the search problem is reduced from the full vocabulary to a small
interval.

Figure~\ref{fig:argmax-saturation} confirms this directly. We intervene on
which token the first attention attends to on the query side and measure which key token
the second attention attends to most strongly, for a current token of value $250$, averaged
over 23~seeds, $\pm 1$ std shaded (number 250 is arbitrary here and can be substituted with other numbers). The key finding is that the second attention's
most-attended key always lies between the current token and the first attention's
target, never exceeding the upper bound provided by the first attention. The curve is also approximately monotonic: redirecting the first attention toward larger tokens causes the second attention to attend to larger keys.
%%%
Furthermore, the first attention's target is pushed far above the current token, the curve interestingly
\textbf{saturates}, where the second attention's most-attended key caps at roughly $300$ regardless of how large the first attention's target becomes: The model has learned to bound its trust in the upper-bound signal: if the first attention reports a target far above the current token (an out-of-distribution signal), the second attention ignores it and falls back on the
local neighborhood. The second attention's QK scores are also visibly smoother than the
first attention's scores within their respective windows
(Appendix~\ref{app:smoothness}), reflecting the benefit of the narrower search
range. The analysis above assumes the first attention is fully concentrated on a single
token; when it splits its weight equally among $n \in \{2,3,4\}$ tokens
separated by~$\delta$, the same band structure persists with only a slight
shift of the argmax toward larger key values as $\delta$ grows, and the argmax
is biased toward the smallest token in the attended set rather than the mean,
ensuring the mechanism remains functionally correct even under distributed
attention (Appendix~\ref{app:split-attn1}).

\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/argmax_saturation_z250_avg_seeds.png}
    \phantomcaption
    \label{fig:argmax-saturation}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/new_fig3b_nkeys_N256_K16.pdf}
    \phantomcaption
    \label{fig:attn-nkeys-vs-seqlen}
  \end{subfigure}

  \caption{\textbf{(a)} The key token that the second attention attends to most strongly as a function of the token that the first attention is intervened to attend to, averaged over seeds and input tokens. The second attention's focus typically lies between the current token and the first attention's target, increases approximately monotonically, and saturates for large first attention targets. In particular, for small interventions, resembling when the next token is very close in value to the current token, which is more common at extreme input lengths, this property does not hold. \textbf{(b)}~Average number of keys with attention weight ${>}0.04$ for varying sequence length for a two-stage and single-stage model. In two-stage models, second-layer attention dominates for wider gaps, while first-layer attention directly determines the output for very small gaps. Consequently, as sequence length increases OOD, the responsible attention maintains a smaller candidate set than the always-responsible first-layer attention in single-stage models.}
  \label{fig:saturation-and-nkeys}
\end{figure}

%%
\textbf{Empirical consequences: smaller candidate sets.}
The windowed monotonicity mechanism has a direct empirical signature in the
attention distributions. Figure~\ref{fig:attn-nkeys-vs-seqlen} shows that,
across all sequence lengths, the second attention attends to fewer keys.
At an attention threshold of $0.04$ and the training
length $K{=}32$, the first attention attends to ${\approx}1.5$--$3$ keys with an average
numerical distance of $2$--$14$, while the second attention attends to $1.2$--$2.2$ keys with
distance $0.3$--$3$. 
%%
%%
As we showed previously, in two-stage models, the second-layer attention is responsible for specifying the output logit based on the hint from the first layer for wider gaps, whereas for very small gaps, the first layer can directly specify the output logit without involving the second layer.
%%
This means that second-layer attention is more responsible for input sequences of moderate length, where small-gap consecutive numbers are less likely to occur, whereas first-layer attention becomes more responsible for very long random sequences, where small gaps are more likely. In line with this, we observe that as the sequence length grows beyond the training distribution, the candidate set associated with the more responsible attention remains smaller than the candidate set of the first-layer attention in the single-stage model, where the first-layer attention is always the responsible one. This is in particular aligned with our observation on length-generalizability of single-stage vs two-stage models in Figure~\ref{fig:three-tasks}.
%This means second layer attention is more responsible in input sequences with not too high lengths which is less likely to produce small-gap consecutive numbers, versus first-layer attention is more responsible for very large random sequences which is more likely to have small gaps. In this regard, we observe that as the sequence length grows out of the training distribution, the size of the candidate set for the attention that is more responsible is smaller than the the size of the candidate set for the first layer attention in the single-stage model (which is always the responsible attention in single-stage models).


As the sequence length grows well beyond training, the responsible attention for the output in the 
two-stage model, namely the first layer attention for  remains tight, while the single-stage model's
attention becomes increasingly diffuse. This tighter focus is a direct
consequence of the band mechanism: the second attention searches a narrow window and can
therefore afford a sharper distribution.

%\nathan{If we are arguing that larger candidate sets at larger lengths are why we length generalize poorly, we should have an experiment showing that larger candidate sets are correlated with poor performance. Otherwise, the argument is incomplete.} \nathan{Adding this experiment shortly.}\khasha{see the red paragraph i wrote above, also in the caption of the candidate-set figure}

\paragraph{Seed-to-seed variation in specialization.}
The degree of cross-layer specialization varies across seeds. For some seeds,
removing the second attention at gap~$1$ still causes an accuracy drop
(Figure~\ref{fig:removal_of_l2_by_gap}), indicating that these seeds rely on
the second layer even at small gaps. This diversity suggests that multiple
valid solutions exist within the two-stage family, differing in the extent to
which the two layers share responsibility at small gaps.


==> sections/related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Transformer sorting and length-generalization}

Prior work studies sorting as a canonical algorithmic task for transformers and situates it within the broader problem of length-generalization. Tracr shows that transformers can be constructed to implement symbolic algorithms, including sorting, providing a useful idealized baseline for mechanistic study \citep{lindner2023tracr}. Empirically, however, whether trained transformers generalize such algorithms depends strongly on inductive biases: \citet{kazemnejad2023impact} show that positional encoding has a major effect on length-generalization. More broadly, \citet{zhou2023algorithms} propose the RASP-Generalization Conjecture, which predicts that transformers tend to length-generalize when a task admits a short RASP-L program that works for all input lengths. Our results suggest a complementary complication: even when such solutions exist, training need not reliably recover the same one, and different learned algorithms can have different length-generalization behavior. \citet{awasthi2023improving} gives a theoretical construction of a two-layer transformer that performs sorting. While these works help answer the question of whether transformers \emph{can} length-generalize, our work focuses on the analysis of what models learn in practice, studying internal mechanisms of learned algorithms, what drives the model to converge to different solutions, and how to control this process.

\subsection{Mechanistic analysis and multiple learned solutions}

\nathan{To mention here in related work: "(How) Do Language Models Track State?"(https://arxiv.org/pdf/2503.02854)}

\nathan{Cite "Random Scaling of Emergent Capabilities
" (https://arxiv.org/abs/2502.17356)}

\citet{huang2026discovering} show that length-generalizing transformers often admit compact, interpretable RASP subprograms that suffice for their behavior, providing direct evidence that trained models can internally implement simple algorithmic programs. \citet{urdshals2025structure} study how internal structure develops in a list-sorting transformer during training, identifying emergent head specializations shaped by the data, but don't study the behavior in more complex, multiple layer models, or study length-generalization.

A separate line of work asks whether models trained on the same task converge to a single mechanism or to multiple distinct solutions. \citet{zhong2023clock} argue that even simple tasks can admit qualitatively different mechanistic solutions, while recent follow-up work argues that some of these apparent differences may be different weight/neuron instantiations of the same underlying algorithm, which is reflected in the underlying geometry \citep{moisescu2025geometry}. Recent work provides further evidence towards a lack of universality across algorithms that transformers implement, showing that transformers can learn various algorithms for simulating mixtures of Markov chains \citep{park2024competition} and analyzing why different strategies may emerge from a bayesian perspective \citep{wurgaft2025context}.

\section*{Acknowledgments}

We thank Cameron S. Allen and Guanghao Ye for helpful discussions early in the project and Stuart J. Russell for feedback. We also thank Shan Chen for assistance in the design and execution of initial experiments.

\section*{Author Contributions}

\textbf{KG} started the project performing an in-depth mechanistic analysis of the single-stage sorting solution. \textbf{NH} found that there was more than one solution type transformers learned depending on the random seed, and \textbf{KG} and \textbf{NH} worked to characterize and analyze the solution types, with specific contributions outlined below.
\textbf{NH} identified the relevance of token gap size, finding adversarial examples in single-stage models and discovering the layer-wise specialization to different gap sizes in two-stage models (Figures \ref{fig:specialization_across_layers}, \ref{fig:removal_of_l2_by_gap}). 
%\textbf{KG} and \textbf{NH} studied what factors affect which solution type emerges (\textbf{NH} Appendix \ref{app:init_scale} and Figure \ref{fig:varN}, \textbf{KG} Figure \ref{fig:varE}). \nathan{KH's proposed rephrasing is missing important nuance in how things happened and also excluding work that I did.}
\textbf{NH} led the study of what factors affect which solution type emerges, studying how one can control which model emerges based on the initialization (Figure \ref{fig:steering_figure}) and other factors impacting which solution emerges (Appendix \ref{app:init_scale} and Figure \ref{fig:varN}). \textbf{KH} later contributed to this exploration studying the impact of embedding sizes in Figure \ref{fig:varE}. 
\textbf{NH} also discovered related phenomena across a broader set of tasks possible with a single layer (Section \ref{sec:alternate_algorithms}) and found generalized results in the setting of training on models with more than 2 layers (Appendix \ref{app:4-layer-section}).

\textbf{KG} designed the hijacking experiments (Figure \ref{fig:hijack-fl-avg}), which causally characterized how direct first-layer circuits and first-to-second-layer hinting circuits contribute separately and jointly to the output, extending and corroborating \textbf{NH}'s observations of these distinct computational routes. \textbf{KG} also discovered a mechanism by which the first layer can provide hints to the second to search in a smaller space, termed the windowed monotonicity mechanism (Figure \ref{fig:argmax-saturation}, Section \ref{sec:attn2-qk-mechanism}), providing an explanation for the second layer having more accurate attention probabilities than the first in some settings, initially identified by \textbf{NH}.
%(\nathan{It is not correct to say that this was identified independently by \textbf{NH} and \textbf{KG} because \textbf{NH} had shown \textbf{KG} these results long before the time \textbf{KG} claims he had first found this result}).
% \nathan{NOTE: the above comment was not responded to neither in the slack nor Overleaf after over 2 weeks, despite other things being responded to, so it is assumed that it is not contested.}
\textbf{KG} also carried out additional mechanistic-interpretability analyses including on the size of the concentration (candidate) sets of the attention mass (Figure \ref{fig:attn-nkeys-vs-seqlen}), and the role of MLPs in shaping the input embeddings in the residual stream to be used by the attentions, where more detail can be found in Appendix Sections C–G. 

\textbf{CS} contributed to the length-generalization experiments and played a substantial role in the early experimental design, framing, and presentation of the paper. All authors contributed to the writing of the manuscript.

\iffalse
\nathan{Initial proposal from Nathan below:}

\textbf{KG} started the project performing an in-depth mechanistic analysis of the single-stage sorting solution. \textbf{NH} found that there was more than one solution type transformers learned depending on the random seed, and \textbf{KG} and \textbf{NH} worked together to characterize and analyze the solution types. \textbf{NH} identified the relevance of token gap size, finding adversarial examples in single-stage models and discovering the layer-wise specialization in two-stage models, and studied what factors affect which solution type emerges. \textbf{NH} also discovered related phenomena across additional tasks and found generalized results in the setting with more than 2 layers. \textbf{KG} identified and investigated the windowed monotonicity mechanism, designed the hijacking experiments, and carried out the additional mechanistic-interpretability analyses, where more detail can be found in Appendix Sections C–G. \textbf{CS} contributed to the length-generalization experiments and played a substantial role in the early experimental design, framing, and presentation of the paper. All authors contributed to the writing of the manuscript.

\nathan{Proposal from Khashayar below (we are in the process of resolving disagreements about what was written below):}

\textbf{KG} started the project performing an in-depth mechanistic analysis of the single-stage sorting solution. \textbf{NH} found that there was more than one solution type transformers learned depending on the random seed, and \textbf{KG} and \textbf{NH} worked together to characterize and analyze the solution types. 
\textbf{KG} realized that second layer attention becomes sharper in type 2 models, and he discovered the mechanism by which this sharpening happens: the attention of the second layer uses a hint provided by the attention of the first layer to search in a smaller space. 
\textbf{NH} identified the relevance of token gap size, finding adversarial examples in single-stage models and discovering the layer-wise specialization to different gap size in two-stage models.
\textbf{KG} did a full mechanistic interpretability of the two type models (\nathan{noting that we agreed to remove this first clause for the next version of the contribution statement}), where he discovered another class of direct circuits from the first layer contributing to the output logits, independent of the first-to-second layer hint circuits.
 \textbf{NH} studied what factors affect which solution type emerges and \textbf{NH} also discovered related phenomena across additional tasks and found generalized results in the setting with more than 2 layers. \textbf{KG} identified and investigated the windowed monotonicity mechanism, and designed the hijacking experiments for type 2 models which revealed the effectiveness and connection of the discovered classes  of circuits for different input positions and gaps. \textbf{KG} also carried out additional mechanistic-interpretability analyses including on the size of the concentration (candidate) sets of the attention mass, and the role of MLPs in shaping the input embeddings in the residual stream to be used by the attentions, where more detail can be found in Appendix Sections C–G. 
\textbf{CS} contributed to the length-generalization experiments and played a substantial role in the early experimental design, framing, and presentation of the paper. All authors contributed to the writing of the manuscript.
\fi

==> sections/setup.tex <==
\section{Setup of the Sorting Task} \label{sec:setup}

%\nathan{Perhaps let's rename this section to set up of the sorting task}

\textbf{Task.} The input to the model is a sequence of $K$ integers drawn uniformly at random (without replacement) from a vocabulary $\{1, \dots, N\}$, followed by a special separator token \texttt{SEP}. The model must then autoregressively predict the sorted sequence, outputting tokens from smallest to largest one at a time. We train on sequences of length $K = 16$ and evaluate length-generalization on lengths $K \in \{2, 3, 4, \dots, N\}$, where $N$, the vocabulary size, is the maximum possible length of a sequence of integers sampled without replacement.

\textbf{Architecture.} We use a two-layer, causally-masked transformer in the style of nanoGPT, simplified to one attention head per layer to facilitate mechanistic analysis. Crucially, we omit positional encodings (NoPE \cite{kazemnejad2023impact}), which is a necessary condition for length-generalization on algorithmic tasks as any model that encodes absolute position is structurally prevented from generalizing to sequences longer than those seen during training. Furthermore, in our preliminary experiments, we observed that positional embeddings induce more complicated difficult-to-interpret algorithms, with each token attending to itself in a manner that nonetheless becomes mechanistically necessary for accurate model performance. For these reasons, we train and analyze models without positional encodings.
%Furthermore, in our early experiments we observed that having positional embedding creates an uninterpretable attention score for each token on itself which nevertheless becomes mechanistically necessary for the model to operate accurately. Due to these reasons, we train and analyze models without positional encodings.  \nathan{Would be good to cite something here, or say a bit more.}.

\textbf{Training.} We train online, sampling a new batch of sequences at each iteration. Due to the large space of possible sequences, it is very unlikely to revisit the same input twice, making the distinction between training data and test data on the same sequence lengths not meaningful. We use the AdamW optimizer with a learning rate of $0.03$ and a batch size of $4096$, optimizing cross-entropy loss over the output tokens. Models reach $100\%$ training accuracy early in training; we then continue training for a total of $60{,}000$ iterations to near-zero loss.


==> sections/steering.tex <==
\section{What Determines Which Algorithm Emerges?}\label{sec:steering}
\subsection{Steering via Initialization Scale}

The results so far show that at least two mechanistically distinct solutions coexist
in the same loss landscape, with fundamentally different length-generalization behavior, with the initialization seed determining
which one is converged to. If the goal is a model that length-generalizes, one must either train many models and select the generalizing one post hoc, or find a way to bias training toward the desired solution. We show that adjusting the relative initialization scale between the two layers is sufficient to do the latter, enabling the steering of nearly all models towards a pre-specified solution type.

\paragraph{Asymmetric initialization steers solution selection.}
We fix one layer's weight initialization standard deviation at $\sigma=0.01$ (a reasonable default) and perturb the other by a small amount: $\Delta \in \{-0.002, -0.001, 0, +0.001, +0.002, +0.003\}$, where positive $\Delta$ means the second layer's weights are initialized at larger scale than the first layer's. For each condition, we train with 100 initialization seeds each and report the proportion of models whose accuracy after ablating the second attention is $\approx 0$ (single-stage models) and the proportion of models whose accuracy after ablating the second attention is $\approx 1$ (two-stage models).

The top panel of Figure~\ref{fig:steering_figure} shows the result:
at the symmetric baseline ($\Delta = 0$), 26\% of models learn the
two-stage solution. Increasing Layer~2's initialization scale to just
$\sigma_2 = 0.013$ ($\Delta = +0.003$) drives this to 100\%. Conversely, increasing Layer~1's scale to $\sigma_1 = 0.012$ ($\Delta = -0.002$) drives it to 0\%. One intuition that could describe this behavior is that initialization scale affects the initial gradients and activations, allowing the layer with larger initialization to develop structure earlier in training. Thus, it could be that when the second layer is initialized as larger, it begins contributing meaningfully before the first layer has the chance to solve the task alone, and the network settles into a compositional solution utilizing both layers. When the first layer is initialized to be larger, one intuition could be that it learns to solve the task before the second layer ever gets involved, which is consistent with the observation that in single-stage models, the second attention layer almost never attends to the token that the model predicts as the next token, suggesting that it was never under gradient pressure to become useful.

\paragraph{Steering has a small cost to length-generalization.}
The bottom panel of Figure~\ref{fig:steering_figure} shows length
generalization curves for all models in each condition, colored by solution type. At a qualitative level, two-stage models (blue) generalize, while single-stage models (red) do not, regardless of the difference in initial scale $\Delta$. However, we find a surprising sensitivity to relative initialization scale in that once the initialization of the second layer initialization is too strong, the model occasionally exhibits less cross-layer specialization (see Figure~\ref{fig:oversteering}), and has poorer length-generalization.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/combined_steering_and_lengthgen.pdf}
    \caption{\textbf{Top:} Fraction of seeds converging to the two-stage solution as a function of the relative initialization scale difference $\Delta = \sigma_2 - \sigma_1$ (sequence length 16, vocabulary size 128, 100 seeds). A small positive $\Delta$ drives all seeds to the two-stage solution and a small negative $\Delta$ drives all seeds to the single-stage solution. \textbf{Bottom:} Length-generalization curves for all models in each condition, colored by solution type. \textcolor{blue}{Two-stage} models generalize beyond the training length, while \textcolor{red}{single-stage} models do not.}
    \label{fig:steering_figure}
\end{figure}

\subsection{Task difficulty biases which solution emerges}
\label{sec:task-difficulty}

We find that the proportion of seeds that converge to each solution type can depend on aspects of the task. In particular, we vary the vocabulary size~$N$ while holding all other hyperparameters constant and measure the fraction of seeds that converge to each solution type across 100 seeds per vocabulary size.

In Figure~\ref{fig:varN}, we see that as the vocabulary size increases, a greater proportion of seeds converge to the two-stage solution. At a vocabulary size of 64, nearly all seeds converge to single-stage solutions, while at vocabulary size 512, the majority converge to two-stage solutions.

One interpretation is that larger vocabulary sizes create a harder discrimination problem: with more possible token values, consecutive elements in the sorted output are closer together in the embedding space, potentially making it more difficult for a single attention layer to reliably identify the correct next token. Under this pressure, the network may be incentivized to use more compositional solutions, recruiting the second layer.

\subsection{Model capacity and emerging solutions}
\label{sec:model-capacity}

Model capacity should act in the opposite direction to task difficulty. In higher embedding dimension~$E$ the token representations have more mutually near-orthogonal directions available, so the query--key inner products that order the candidate tokens can be realized at smaller embedding norm. Since the weights begin at a small initialization scale, a solution expressible at smaller norm is easier for the optimizer to reach, and increasing~$E$ should therefore favor the single-stage solution.

We vary~$E$ with the task fixed at vocabulary size $N = 256$ and sequence length $K = 16$, estimating each width from a common sample of $70$ seeds that learned the task. Figure~\ref{fig:varE} confirms the prediction: the two-stage share falls from every trained seed at $E = 32$ to none at $E = 80$, crossing even odds between $E = 60$ and $E = 62$. The trend is opposite to that of vocabulary size, suggesting that what selects the algorithm is the difficulty of the task relative to the capacity available to meet it.


==> sections/two_algorithms.tex <==
\section{Two Sorting Algorithms Emerge from Initialization}
\label{sec:two-algorithms}

Across different initializations of weights, with the training data and its ordering held fixed, we find that trained two-layer transformers achieving perfect sorting accuracy do not all learn the same algorithm. Figure \ref{fig:three-tasks} shows that when the second attention layer is removed from the trained model, per-seed accuracy splits into two tight clusters: one cluster that retains full sample accuracy, and another cluster of seeds where the accuracy is tightly clustered around 0. This is in contrast to the first attention layer, which can't be removed for any seed without dropping the sample accuracy to 0. The fact that the sample accuracy after ablating the second attention is approximately a Bernoulli random variable suggests that there are at least two qualitatively different algorithms that emerge from training, depending on the weight initialization.

We call the algorithm type that does not depend on the second attention a \textbf{single-stage solution}, and the algorithm type that does depend on the second attention \textbf{a two-stage solution}. The distinction between these two solution types has a striking consequence for length-generalization, as two-stage solutions generalize to sequences longer than those seen during training, while single-stage solutions do not (Figure~\ref{fig:three-tasks}). The remainder of this section describes the single-stage solution at a high level. Section~\ref{sec:mechanistic} then describes how the two-stage solution is different and provides a mechanistic account of why the two-stage solution length-generalizes.

\subsection{Single-stage solutions.}

In single-stage solutions, there is only one attention layer that becomes involved in the computation, and therefore only one query per position to consider. We denote the full sequence (for $k=16$) as
$$x_1, \dots, x_{16}, \texttt{SEP}, x_{s(1)}, \dots, x_{s(16)},$$
where $x_1, \dots, x_{16}$ is the unsorted input and $s$ is the permutation that sorts it, so that $$x_{s(1)}  < x_{s(2)} < \dots < x_{s(16)}.$$

When token $x_{s(i)}$ is the query, the model must predict $x_{s(i+1)}$ as the next token, except for when the separator token is the query, in which the model must predict $x_{s(1)}$. We also denote the "gap" between consecutive tokens at token $i$ as $g_i := x_{s(i+1)} - x_{s(i)}$, which we discuss as relevant to two-stage solutions in Section~\ref{sec:specialization}.

We find that the query at position $x_{s(i)}$ attends most strongly to the position holding $x_{s(i+1)}$ in the unsorted part of the sequence, but also attends partially to positions holding larger values (Figure~\ref{fig:ridgeline}, bottom). The resulting value vector is therefore a linear combination of nearby tokens in sorted order, typically concentrated on the correct one. However, in instances where token attended to most is not the correct next token, the transformer still predicts a correct next token. We hypothesize that the role of the first attention in the single-stage model is to select a set of potential next tokens, which we term the candidate set, consisting of those assigned non-trivial attention probability by the attention. We further hypothesize that the two MLP layers and the unembedding matrix could be thought of as selecting among this candidate set of tokens to produce the correct output.


\section{Two-stage solutions and their Mechanistic Analysis}
\label{sec:mechanistic}
%\subsection{Two-stage solutions.}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{arxiv/figures/fig2_single_sample_heatmap_60k.pdf}
    \caption{Attention probability heatmaps for a two-stage seed (top) and a single-stage seed (bottom), with tokens ordered by numerical value. Both layers of the two-stage model more reliably attend to the correct next token, whereas the single-stage model's first layer distributes attention across a broader set of nearby candidate tokens. In this example, while the two-stage layers have similar candidate-set sizes, which layer is sharper varies with sequence length (Figure~\ref{fig:attn-nkeys-vs-seqlen}), but the second layer is always attends more accurately than the first.}
\label{fig:ridgeline}
\end{figure}

